Spectral geometry over the disk : Weyl's law and nodal sets

In this M.Sc. thesis (Universit\'e de Montr\'eal, 2007), we consider problems arising in the study of the spectrum of the Dirichlet Laplacian on a disk as well as on a circular sector. The first part of the thesis is concerned with the location of the nodal line of the second eigenfunction of a sector. In the second part of the thesis we develop an efficient algorithm for ordering the eigenvalues of a disk, and study numerically the growth of the error term in Weyl's law. We also give a detailed proof of a theorem due to Kuznetsov and Fedosov (1965), who obtained a van der Corput type estimate on the remainder. The result of Kuznetsov and Fedosov was rediscovered in 2011 by Y. Colin de Verdi\`ere using similar techniques, see http://arxiv.org/pdf/1104.2233v2.pdf .

==> acknowledgement.tex <==
\chapter*{Acknowledgement}

For those who are fine with me.


==> layout.tex <==

\hoffset = 0pt

\voffset = 0pt

\oddsidemargin = 0pt

\evensidemargin = 0pt

\headheight = 18pt
% attention on est en "landscape"
%\textheight = 6.5in

\textheight = 8.0in

\marginparsep = 0pt

\footskip = 55pt
% attention on est en "landscape"
%\paperwidth = 11in

\paperwidth = 8.5in

\topmargin = 0pt

\headsep = 19pt
% attention on est en "landscape"
%\textwidth = 9in

\textwidth = 6.5in

\marginparwidth = 0pt

\marginparpush = 0pt
% attention on est en "landscape"
%\paperheight = 8.5in

\paperheight = 11in


==> macro.tex <==
% corollaire
\theoremstyle{break} \theorembodyfont{\upshape}
\newtheorem{Cor}{\textbf{Corollaire}}[section]

% example
\theoremstyle{break} %\theorembodyfont{\fontfamily{crm}\selectfont}
\newtheorem{Exa}{Exemple}[section]

% remarque
\theoremstyle{break} \theorembodyfont{\itshape}%\theorembodyfont{\fontfamily{crm}\selectfont}
\newtheorem{Rem}{\textbf{Remarque}}[section]

% lemme
\theoremstyle{break} \theorembodyfont{\upshape}
\newtheorem{Lem}{\textbf{Lemme}}[section]

% définition
\theoremstyle{break} \theorembodyfont{\upshape}
\newtheorem{Def}{\textbf{Définition}}[section]

% théorème
\theoremstyle{break} \theorembodyfont{\upshape}
\newtheorem{Thm}{\textbf{Théorème}}[section]

% doit être utilisé seulement une fois pour tous les différents types de "theorems environment"
\theoremheaderfont{\upshape}

%%% trucs pour divers types de convergences

\newcommand{\cvp}{\stackrel{\mathbf{P}}{\to}}
\newcommand{\cvps}{\stackrel{p.s.}{\to}}
\newcommand{\cvd}{\stackrel{\mathcal{D}}{\to}}
\newcommand{\pardef}{\stackrel{def}{=}}
\newcommand{\eqas}{\stackrel{p.s}{=}}

